Event disturbance rejection: a case study

This article introduces the problem of robust event disturbance rejection. Inspired by the design principle of linear output regulation, a control structure based on excitable systems is proposed. Unlike the linear case, contraction of the closed-loop system must be enforced through specific input signals. This induced contraction enables a steady-state analysis similar to the linear case. Thanks to the excitable nature of the systems, the focus shifts from precise trajectory tracking to the regulation of discrete events, such as spikes. The study emphasizes rejecting events rather than trajectories and demonstrates the robustness of the approach, even under mismatches between the controller and the exosystem. This work is a first step towards developing a design principle for event regulation.

==> tikz_diagrams/tikz_settings.tex <==
%\tikzset{
%block/.style={
%  draw,
%  fill=white!20,
%  rectangle,
%  minimum height=3em,
%  minimum width=6em
%  },

%sum/.style={
%  draw,
%  fill=white!20,
%  circle,
%  },


\tikzset{
output/.style ={coordinate},
input/.style = {coordinate}
}

\tikzset{
}


\tikzstyle{neuron} = [
circle,
minimum size=0.75cm,
color=black,
fill=black!5,
draw=black,
inner sep=1pt,
line width=0.5pt
]

\tikzstyle{synapse} = [
ellipse,
minimum width=0.8cm,
minimum height=0.6cm,
rounded corners=0pt,
align=center,
color=black,
fill=black!5,
draw=black,
inner sep=0.5pt,
line width=0.5pt
]

\tikzstyle{sum} = [
fill=white!20,
circle,
inner sep = 0pt,
outer sep = 0pt,
minimum width=0.05cm,  % Smaller width
minimum height=0.05cm,  % Smaller height
anchor=center
]

\tikzstyle{block1} = [
draw,
color=black,
fill=black!5,
rectangle,
rounded corners=0pt,
minimum height=0.75cm,
minimum width=1cm,
% text width=2.5cm,
line width=0.5pt,
anchor = west,
align = center,
text=black,
inner sep=0pt
]

\tikzstyle{block} = [
draw,
color=black,
fill=black!5,
rectangle,
rounded corners=0pt,
minimum height=0.75cm,
minimum width=1.5cm,
% text width=2.5cm,
line width=0.5pt,
anchor = west,
align = center,
text=black,
inner sep=2pt
]

\tikzstyle{lines} = [
black,
line width=0.5pt,
->
]

==> tikz_settings.tex <==
\tikzset{
block/.style={
  draw, 
  fill=white!20, 
  rectangle, 
  minimum height=3em, 
  minimum width=6em
  },
sum/.style={
  draw, 
  fill=white!20, 
  circle, 
  },
input/.style={coordinate},
output/.style={coordinate},
pinstyle/.style={
  pin edge={to-,thin,black}
  }
}

\tikzstyle{neuron} = [
circle, 
minimum size=1cm,
draw=black]
